Communication-Efficient Federated Distillation

Communication constraints are one of the major challenges preventing the wide-spread adoption of Federated Learning systems. Recently, Federated Distillation (FD), a new algorithmic paradigm for Federated Learning with fundamentally different communication properties, emerged. FD methods leverage ensemble distillation techniques and exchange model outputs, presented as soft labels on an unlabeled public data set, between the central server and the participating clients. While for conventional Federated Learning algorithms, like Federated Averaging (FA), communication scales with the size of the jointly trained model, in FD communication scales with the distillation data set size, resulting in advantageous communication properties, especially when large models are trained. In this work, we investigate FD from the perspective of communication efficiency by analyzing the effects of active distillation-data curation, soft-label quantization and delta-coding techniques. Based on the insights gathered from this analysis, we present Compressed Federated Distillation (CFD), an efficient Federated Distillation method. Extensive experiments on Federated image classification and language modeling problems demonstrate that our method can reduce the amount of communication necessary to achieve fixed performance targets by more than two orders of magnitude, when compared to FD and by more than four orders of magnitude when compared with FA.

==> Communication-Efficient Federated Ensemble Distillation/lang_model_results/fig_distilbert_results_sst2_and_agnews_100.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.485\textwidth}
        \centering
        \includegraphics[width=1.\linewidth]{lang_model_results/sst2_accuracy_vs_communication_cost_fd_fa_distillsamples_1000.pdf}
        \caption{SST2.}
        \label{fig:distilbert_results_sst2_100}
    \end{subfigure}
    \begin{subfigure}[b]{0.485\textwidth}
        \centering
        \includegraphics[width=1.\linewidth]{lang_model_results/ag_news_accuracy_vs_communication_cost_fd_fa_distillsamples_1000.pdf}
        \caption{AG-News.}
        \label{fig:distilbert_results_agnews_100}
    \end{subfigure}
    \caption{DistilBERT model performance as a function of communicated bits for our proposed CFD method and baselines FA and FD. This model was evaluated on the SST2 and AG-News datasets, with $\alpha$ = 100.0 and 1.0, using 100\% of the disitillation dataset samples (10 clients with 100\% participation rate).}
    \label{fig:distilbert_results_sst2_and_agnews_100}
\end{figure}

==> Communication-Efficient Federated Ensemble Distillation/lang_model_results/fig_distilbert_results_sst2_and_agnews_50_20_10.tex <==
\begin{figure*}[!ht]
    \centering
    % ------------------------------------------------------------------------------------------------------------
    % Distillation samples: 50%
    % ------------------------------------------------------------------------------------------------------------
    \begin{subfigure}[b]{0.485\textwidth}
        \centering
        \includegraphics[width=1.\linewidth]{lang_model_results/sst2_accuracy_vs_communication_cost_fd_distillsamples_500.pdf}
        \caption{SST2 (50\% distillation data samples).}
        \label{fig:distilbert_results_sst2_50}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.485\textwidth}
        \centering
        \includegraphics[width=1.\linewidth]{lang_model_results/ag_news_accuracy_vs_communication_cost_fd_distillsamples_500.pdf}
        \caption{AG-News (50\% distillation data samples).}
        \label{fig:distilbert_results_agnews_50}
    \end{subfigure} 
    \newline~\newline
    % ------------------------------------------------------------------------------------------------------------
    % Distillation samples: 20%
    % ------------------------------------------------------------------------------------------------------------
    \begin{subfigure}[b]{0.485\textwidth}
        \centering
        \includegraphics[width=1.\linewidth]{lang_model_results/sst2_accuracy_vs_communication_cost_fd_distillsamples_200.pdf}
        \caption{SST2 (20\% distillation data samples).}
        \label{fig:distilbert_results_sst2_20}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.485\textwidth}
        \centering
        \includegraphics[width=1.\linewidth]{lang_model_results/ag_news_accuracy_vs_communication_cost_fd_distillsamples_200.pdf}
        \caption{AG-News (20\% distillation data samples).}
        \label{fig:distilbert_results_agnews_20}
    \end{subfigure}
    \newline~\newline
    % ------------------------------------------------------------------------------------------------------------
    % Distillation samples: 10%
    % ------------------------------------------------------------------------------------------------------------
    \begin{subfigure}[b]{0.485\textwidth}
        \centering
        \includegraphics[width=1.\linewidth]{lang_model_results/sst2_accuracy_vs_communication_cost_fd_distillsamples_100.pdf}
        \caption{ SST2 (10\% distillation data samples). }
        \label{fig:distilbert_results_sst2_10}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.485\textwidth}
        \centering
        \includegraphics[width=1.\linewidth]{lang_model_results/ag_news_accuracy_vs_communication_cost_fd_distillsamples_100.pdf}
        \caption{AG-News (10\% distillation data samples).}
        \label{fig:distilbert_results_agnews_10}
    \end{subfigure}
    % ------------------------------------------------------------------------------------------------------------
    \caption{Communication efficiency (i.e., accuracy vs communication cost) for Federated Learning of DistilBERT, on the SST2 and AG-News datasets, with $\alpha$ = 100.0 and 1.0, using 50\%, 20\%, and 10\% of the disitillation dataset samples (10 clients with 100\% participation rate).}
    \label{fig:distilbert_results_sst2_and_agnews_50_20_10}
\end{figure*}

==> Communication-Efficient Federated Ensemble Distillation/lang_model_results/table_distilbert_50_20_10_bits_to_target.tex <==
\begin{table*}[!ht]
\caption{Upstream communication measured in [MB], necessary to achieve a specific target accuracy in Federated Learning of DistillBERT, on the SST2 and AG-News data set, at different numbers of distillation data samples (50\%, 20\%, and 10\%), and levels of data heterogeneity ($\alpha$=100.0 and 1.0).}
\centering
\begin{tabular}{llrrrrr}
\toprule
Dataset             & Distillation  & $\alpha$  & FA            & FD        & CFD-1-32       & $\text{CFD}_\Delta$-1-32 \\
(Target Accuracy)   & Dataset Size  &           &               &           &           & \\
\midrule
SST2    & 50\%      & 100.0 & 267.820  & 0.135 & 0.003 & 0.003 \\
(0.88)  &           & 1.0   & 803.460  & 0.404 & 0.004 & 0.005 \\
        & 20\%      & 100.0 & 267.820  & 0.161 & 0.003 & 0.004 \\
        &           & 1.0   & 803.460  & 0.161 & 0.003 & 0.005 \\
        & 10\%      & 100.0 & 267.820  & 0.135 & 0.001 & 0.001 \\
        &           & 1.0   & 803.460  & 0.161 & 0.004 & 0.006 \\
\midrule
AG-News & 50\%      & 100.0 & 535.640  & 0.480 & 0.015 & 0.018 	\\
(0.91)  &           & 1.0   & 1071.280 & 1.920 & 0.071 & 0.084 	\\
        & 20\%      & 100.0 & 535.640  & 0.384 & 0.003 & 0.004 	\\
        &           & 1.0   & 1071.280 & 1.536 & 0.029 & 0.034 	\\
        & 10\%      & 100.0 & 535.640  & 0.384 & 0.007 & 0.009 	\\
        &           & 1.0   & 1071.280 & 0.960 & 0.014 & 0.018 	\\
\bottomrule
\end{tabular}
\label{tab:distilbert_bits_to_target_50_20_10}
\end{table*}

==> Communication-Efficient Federated Ensemble Distillation/lang_model_results/table_distilbert_50_20_10_bits_to_target__.tex <==
\begin{table*}[!ht]
\caption{Upstream communication measured in [MB], necessary to achieve a specific target accuracy in Federated Learning of DistillBERT, on the SST2 and AG-News data set, at different numbers of distillation data samples (50\%, 20\%, and 10\%), and levels of data heterogeneity ($\alpha$=100.0 and 1.0).}
\centering
\begin{tabular}{llrrrrr}
\toprule
Dataset             & Distillation  & $\alpha$  & FA            & FD        & CFD-1-32       & $\text{CFD}_\Delta$-1-32 \\
(Target Accuracy)   & Dataset Size  &           &               &           &           & \\
\midrule
SST2    & 50\%      & 100.0 & 2142.56     & 1.08   & 0.02   & 0.02 \\
(0.88)  &           & 1.0   & 6427.68     & 3.23   & 0.03   & 0.04 \\
        & 20\%      & 100.0 & 2142.56     & 1.29   & 0.02   & 0.03 \\
        &           & 1.0   & 6427.68     & 1.29   & 0.02   & 0.04 \\
        & 10\%      & 100.0 & 2142.56     & 1.08   & 0.01   & 0.01 \\
        &           & 1.0   & 6427.68     & 1.29   & 0.03   & 0.05 \\
\midrule
AG-News & 50\%      & 100.0 & 4285.12     & 3.84    & 0.12  & 0.14 \\
(0.91)  &           & 1.0   & 8570.24     & 15.36   & 0.57  & 0.67 \\
        & 20\%      & 100.0 & 4285.12     & 3.07    & 0.02  & 0.03 \\
        &           & 1.0   & 8570.24     & 12.29   & 0.23  & 0.27 \\
        & 10\%      & 100.0 & 4285.12     & 3.07    & 0.06  & 0.07 \\
        &           & 1.0   & 8570.24     & 7.68    & 0.11  & 0.14 \\
\bottomrule
\end{tabular}
\label{tab:distilbert_bits_to_target_50_20_10}
\end{table*}

==> Communication-Efficient Federated Ensemble Distillation/lang_model_results/table_distilbert_bits_to_target.tex <==
\begin{table*}[]
\caption{Upstream and downstream communication, measured in [MB], required in Federated Training of DistilBERT, to achieve a specific target accuracy, on the SST-2 and AG-News data sets at different levels of data heterogeneity $\alpha$.}
\centering
\begin{tabular}{llrrrrrrr}
\toprule
Dataset           & $\alpha$ & Up/Down  & FA            & FD        & CFD-1-32  & $\text{CFD}_\Delta$-1-32  & CFD-1-1   & $\text{CFD}_\Delta$-1-1 \\
(Target Accuracy) &          &          &               &           &           &                           &           &                            \\
\midrule
SST2              & 100.0    & Up       & 267.820 	& 0.270 & 0.004  & \textbf{0.005}  & 0.029 & 0.044 \\
(0.88)            & 100.0    & Down     & 267.820 	& 0.270 & 0.269  & 0.269 & \textbf{0.030} & 0.044  \\
                  & 1.0      & Up       & 803.460 	& 0.539 & \textbf{0.007}  & 0.011  & 0.031 & 0.046  \\
                  & 1.0      & Down     & 803.460 	& 0.539 & 0.539  & 0.539 & \textbf{0.034} & 0.050  \\
\midrule
AG-News           & 100.0    & Up       & 535.640 	& 1.920 & \textbf{0.030}  & 0.035  & 0.090 & 0.104  \\
(0.91)            & 100.0    & Down     & 535.640 	& 1.920 & 1.920 & 1.920 & \textbf{0.090} & 0.104  \\
                  & 1.0      & Up       & 1071.280 	& 4.800 & 0.142  & 0.169  & \textbf{0.101} & 0.119  \\
                  & 1.0      & Down     & 1071.280 	& 4.800 & 9.600 & 9.600 & \textbf{0.105} & 0.121  \\
\bottomrule
\end{tabular}
\label{tab:distilbert_bits_to_target}
\end{table*}

==> Communication-Efficient Federated Ensemble Distillation/lang_model_results/table_distilbert_bits_to_target__.tex <==
\begin{table*}[]
\caption{Upstream and downstream communication, measured in [MB], required in Federated Training of DistilBERT, to achieve a specific target accuracy, on the SST-2 and AG-News data sets at different levels of data heterogeneity $\alpha$.}
\centering
\begin{tabular}{llrrrrrrr}
\toprule
Dataset           & $\alpha$ & Up/Down  & FA            & FD        & CFD-1-32  & $\text{CFD}_\Delta$-1-32  & CFD-1-1   & $\text{CFD}_\Delta$-1-1 \\
(Target Accuracy) &          &          &               &           &           &                           &           &                            \\
\midrule
SST2              & 100.0    & Up       & 2142.56     & 2.16    & 0.03    & 0.04                    & 0.23   & 0.35  \\
(0.88)            & 100.0    & Down     & 2142.56     & 2.16    &           &                           & 0.24   & 0.35  \\
                  & 1.0      & Up       & 6427.68     & 4.31    & 0.06    & 0.09                    & 0.25   & 0.37  \\
                  & 1.0      & Down     & 6427.68     & 4.31    &           &                           & 0.27   & 0.40  \\
\midrule
AG-News           & 100.0    & Up       & 4285.12     & 15.36   & 0.24    & 0.28                   & 0.72   & 0.83  \\
(0.91)            & 100.0    & Down     & 4285.12     & 15.36   &           &                           & 0.72   & 0.83  \\
                  & 1.0      & Up       & 8570.24     & 38.40   & 1.14    & 1.35                   & 0.81   & 0.95  \\
                  & 1.0      & Down     & 8570.24     & 38.40   &           &                           & 0.84   & 0.97  \\
\bottomrule
\end{tabular}
\label{tab:distilbert_bits_to_target}
\end{table*}

==> Communication-Efficient Federated Ensemble Distillation/lang_model_results/table_distilbert_pate_bits_to_target.tex <==
\begin{table*}
\caption{Upstream and downstream communication, required by DistilBERT, to achieve a specific target accuracy in a Federated Learning scenario. Specifically, 1-bit quantization ($\mathcal{Q}_1$) was applied in upstream ($b_{up}=1$) and downstream ($b_{down}=1$) communication, and 100\% of the distillation data samples were processed.}
\centering
\begin{tabular}{lllrr}
\toprule
Dataset             & $\alpha$      & Up/Down       & CFD       & $\text{CFD}_\Delta$ \\
(Target Accuracy)   &               &               &           &                     \\
\midrule
SST2                & 100.0         & Up            & 0.23 MB  & 0.35 MB \\
(0.88)              &               & Down          & 0.24 MB  & 0.35 MB \\
                    & 1.0           & Up            & 0.25 MB  & 0.37 MB \\
                    &               & Down          & 0.27 MB  & 0.40 MB \\
\midrule
AG-News             & 100.0         & Up            & 0.72 MB  & 0.83 MB \\
(0.91)              &               & Down          & 0.72 MB  & 0.83 MB \\
                    & 1.0           & Up            & 0.81 MB  & 0.95 MB \\
                    &               & Down          & 0.84 MB  & 0.97 MB \\
\bottomrule
\end{tabular}
\label{tab:distilbert_pate_bits_to_target}
\end{table*}

==> lang_model_results/table_distilbert_50_20_10_bits_to_target__.tex <==
\begin{table*}[!ht]
\caption{Upstream communication measured in [MB], necessary to achieve a specific target accuracy in Federated Learning of DistillBERT, on the SST2 and AG-News data set, at different numbers of distillation data samples (50\%, 20\%, and 10\%), and levels of data heterogeneity ($\alpha$=100.0 and 1.0).}
\centering
\begin{tabular}{llrrrrr}
\toprule
Dataset             & Distillation  & $\alpha$  & FA            & FD        & CFD-1-32       & $\text{CFD}_\Delta$-1-32 \\
(Target Accuracy)   & Dataset Size  &           &               &           &           & \\
\midrule
SST2    & 50\%      & 100.0 & 2142.56     & 1.08   & 0.02   & 0.02 \\
(0.88)  &           & 1.0   & 6427.68     & 3.23   & 0.03   & 0.04 \\
        & 20\%      & 100.0 & 2142.56     & 1.29   & 0.02   & 0.03 \\
        &           & 1.0   & 6427.68     & 1.29   & 0.02   & 0.04 \\
        & 10\%      & 100.0 & 2142.56     & 1.08   & 0.01   & 0.01 \\
        &           & 1.0   & 6427.68     & 1.29   & 0.03   & 0.05 \\
\midrule
AG-News & 50\%      & 100.0 & 4285.12     & 3.84    & 0.12  & 0.14 \\
(0.91)  &           & 1.0   & 8570.24     & 15.36   & 0.57  & 0.67 \\
        & 20\%      & 100.0 & 4285.12     & 3.07    & 0.02  & 0.03 \\
        &           & 1.0   & 8570.24     & 12.29   & 0.23  & 0.27 \\
        & 10\%      & 100.0 & 4285.12     & 3.07    & 0.06  & 0.07 \\
        &           & 1.0   & 8570.24     & 7.68    & 0.11  & 0.14 \\
\bottomrule
\end{tabular}
\label{tab:distilbert_bits_to_target_50_20_10}
\end{table*}

==> lang_model_results/table_distilbert_bits_to_target__.tex <==
\begin{table*}[]
\caption{Upstream and downstream communication, measured in [MB], required in Federated Training of DistilBERT, to achieve a specific target accuracy, on the SST-2 and AG-News data sets at different levels of data heterogeneity $\alpha$.}
\centering
\begin{tabular}{llrrrrrrr}
\toprule
Dataset           & $\alpha$ & Up/Down  & FA            & FD        & CFD-1-32  & $\text{CFD}_\Delta$-1-32  & CFD-1-1   & $\text{CFD}_\Delta$-1-1 \\
(Target Accuracy) &          &          &               &           &           &                           &           &                            \\
\midrule
SST2              & 100.0    & Up       & 2142.56     & 2.16    & 0.03    & 0.04                    & 0.23   & 0.35  \\
(0.88)            & 100.0    & Down     & 2142.56     & 2.16    &           &                           & 0.24   & 0.35  \\
                  & 1.0      & Up       & 6427.68     & 4.31    & 0.06    & 0.09                    & 0.25   & 0.37  \\
                  & 1.0      & Down     & 6427.68     & 4.31    &           &                           & 0.27   & 0.40  \\
\midrule
AG-News           & 100.0    & Up       & 4285.12     & 15.36   & 0.24    & 0.28                   & 0.72   & 0.83  \\
(0.91)            & 100.0    & Down     & 4285.12     & 15.36   &           &                           & 0.72   & 0.83  \\
                  & 1.0      & Up       & 8570.24     & 38.40   & 1.14    & 1.35                   & 0.81   & 0.95  \\
                  & 1.0      & Down     & 8570.24     & 38.40   &           &                           & 0.84   & 0.97  \\
\bottomrule
\end{tabular}
\label{tab:distilbert_bits_to_target}
\end{table*}

==> lang_model_results/table_distilbert_pate_bits_to_target.tex <==
\begin{table*}
\caption{Upstream and downstream communication, required by DistilBERT, to achieve a specific target accuracy in a Federated Learning scenario. Specifically, 1-bit quantization ($\mathcal{Q}_1$) was applied in upstream ($b_{up}=1$) and downstream ($b_{down}=1$) communication, and 100\% of the distillation data samples were processed.}
\centering
\begin{tabular}{lllrr}
\toprule
Dataset             & $\alpha$      & Up/Down       & CFD       & $\text{CFD}_\Delta$ \\
(Target Accuracy)   &               &               &           &                     \\
\midrule
SST2                & 100.0         & Up            & 0.23 MB  & 0.35 MB \\
(0.88)              &               & Down          & 0.24 MB  & 0.35 MB \\
                    & 1.0           & Up            & 0.25 MB  & 0.37 MB \\
                    &               & Down          & 0.27 MB  & 0.40 MB \\
\midrule
AG-News             & 100.0         & Up            & 0.72 MB  & 0.83 MB \\
(0.91)              &               & Down          & 0.72 MB  & 0.83 MB \\
                    & 1.0           & Up            & 0.81 MB  & 0.95 MB \\
                    &               & Down          & 0.84 MB  & 0.97 MB \\
\bottomrule
\end{tabular}
\label{tab:distilbert_pate_bits_to_target}
\end{table*}
